EgoVITA: Learning to Plan and Verify for Egocentric Video Reasoning

Egocentric video understanding requires procedural reasoning under partial observability and continuously shifting viewpoints. Current multimodal large language models (MLLMs) struggle with this setting, often generating plausible but visually inconsistent or weakly grounded responses. We introduce $\textbf{EgoVITA}$, a framework that decomposes egocentric video reasoning into a structured $\textit{plan-then-verify}$ process. The model first generates an $\textbf{egocentric plan}$: a causal sequence of anticipated actions from a first-person perspective. This plan is then evaluated by an $\textbf{exocentric verification}$ stage that uses third-person reasoning over the same video to verify its spatiotemporal and logical consistency, without exocentric video input. This decomposition enables cross-perspective feedback without requiring paired ego-exo supervision. To train this reasoning process, we adopt Group Relative Policy Optimization (GRPO) with two dense reward signals: one that grounds anticipated actions in subsequent visual observations and another that reinforces consistent third-person verification. $\textbf{EgoVITA}$ achieves state-of-the-art performance on egocentric reasoning benchmarks, outperforming Qwen2.5-VL-7B by $\mathbf{+7.7}$ on EgoBlind and $\mathbf{+4.4}$ on EgoOrient, while maintaining strong generalization on exocentric video tasks with only $52k$ training samples.

==> tables/rollout_analysis.tex <==
\begin{table}[t!]
\centering
\caption{\textcolor{blue}{\textbf{Rollout failure analysis.} 3,278 Qwen2.5-VL rollouts tagged by Gemini-3.1-Flash. When \textit{ego\_plan} was incorrect (B+C+D, 993 cases), \textit{exo\_verify} rejected the plan in 69\% of cases (B+D, 681) and confirmed it in only 31\% (C, 312).}}
\label{tab:rollout_analysis}
\vspace{-3mm}
\renewcommand{\arraystretch}{1.1}
\fontsize{6pt}{7pt}\selectfont
\setlength{\tabcolsep}{2mm}
\begin{tabular}{l r r}
\toprule
\textbf{Type} & \textbf{N} & \textbf{\%} \\
\midrule
A. All correct   & 1847 & 56 \\
B. Plan fixed by \textit{exo\_verify}    &  487 & 15 \\
C. Incorrect plan confirmed   &  312 & 10 \\
D. Fix attempted but failed    &  194 &  6 \\
\midrule
E. ACMG noisy ($N{=}16$ window)    &  341 & 10 \\
F. ACMG static feature bias     &   97 &  3 \\
\bottomrule
\end{tabular}
\vspace{-4mm}
\end{table}

